Conditionally Parameterized, Discretization-Aware Neural Networks for Mesh-Based Modeling of Physical Systems

Simulations of complex physical systems are typically realized by discretizing partial differential equations (PDEs) on unstructured meshes. While neural networks have recently been explored for surrogate and reduced order modeling of PDE solutions, they often ignore interactions or hierarchical relations between input features, and process them as concatenated mixtures. We generalize the idea of conditional parameterization -- using trainable functions of input parameters to generate the weights of a neural network, and extend them in a flexible way to encode critical information. Inspired by discretized numerical methods, choices of the parameters include physical quantities and mesh topology features. The functional relation between the modeled features and the parameters is built into the network architecture. The method is implemented on different networks and applied to frontier scientific machine learning tasks including the discovery of unmodeled physics, super-resolution of coarse fields, and the simulation of unsteady flows with chemical reactions. The results show that the conditionally-parameterized networks provide superior performance compared to their traditional counterparts. The CP-GNet - an architecture that can be trained on very few data snapshots - is proposed as the first deep learning model capable of standalone prediction of reacting flows on irregular meshes.

==> bak/1d_diffusion.tex <==
\subsection{1D Diffusion}
For an easier understanding of the idea of conditional parameterization, we first apply it on a extremely basic network -- single layer 1D CNN, and use it to predict a simple problem -- 1D diffusion. The problem is governed by a linear PDE for a scalar variable $u(x,t)$:
\begin{equation}\label{eq diffusion}
\begin{split}
    &\frac{\partial u}{\partial t} - \nu\frac{\partial^2 u}{\partial x^2}=0,\\
    &x\in[0,L], t\in[0,T],\\
    &u(0,t)=u_0, u(L,t)=u_L,\\
    &u(x,0)=0 \text{ for } x\in(0,L)
\end{split}
\end{equation}
where $\nu$ is a constant diffusion coefficient, $L=1$ is the length of domain, and $T=0.1$ is the length of time period studied, $u_0=0, u_L=1$ are two fixed Dirichlet boundary conditions. 

With a forward in time and central in space discretization, the discretized form of \eqr{eq diffusion} is:
\begin{equation}\label{eq diffusion discrete}
    \frac{\Delta u^k_i}{\Delta t}-\nu\frac{u^k_{i-1}-2u^k_i+u^k_{i+1}}{\Delta x^2}=0,
\end{equation}
where $i$ is the grid index, $k$ is the time step index, and $\Delta u^k_i = u^{k+1}_i-u^{k}_i$.

\eqr{eq diffusion discrete} can be re-written into:
\begin{equation}\label{eq diffusion discrete2}
    \Delta u^k_i=C(u^k_{i-1}-2u^k_i+u^k_{i+1}),
\end{equation}
where $C=\nu\frac{\Delta t}{\Delta x^2}$.

Except for $C$, the RHS term of \eqr{eq diffusion discrete2} fits exactly into the form of a 1D convolution operator with a kernel size of 3. Thus we can train a convolution filter $\mathbf{w}\in\re^3$, which by itself forms a single layer CNN, and expect it to model the system perfectly for a fixed $C$ such that:
\begin{equation}\label{eq diffusion conv}
    \Delta \mathbf{u}^{k} = \mathbf{w}*\mathbf{u}^{k},
\end{equation}
where $(*)$ denotes the convolution operation.

The verify this, the problem is solved using \eqr{eq diffusion discrete}, with $\nu=1, \Delta t=\num{5e-5}, \Delta x=0.01$, which leads to $C=0.5$ and 2000 steps in total. The first 50 steps is used for training and prediction is then performed from the initial condition for the full time period. The results are shown in Fig.~\ref{fig diffusion C0.5}, where the model reached machine zero. 

However, when $C$ changes, the above model will not be able to be predictive because the parameters are overfitted to the single training case. This is demonstrated one a new case with $\Delta x=0.02$ and the rest parameters remain unchanged, which leads to $C=0.125$. As shown in Fig.~\ref{fig diffusion C0.125}, the CNN overshoots the diffusion speed because it is trained for $C=0.5$, which on this combination of $\Delta x$ and $\Delta t$ will be equivalent to a 4X larger $\nu$.

For this linear case, this limitation can be easily addressed by making $\mathbf{w}$ a linear function of $C$, and the conditionally parameterized version of \eqr{eq diffusion conv} is:
\begin{equation}\label{eq diffusion cpconv}
    \Delta \mathbf{u}^{k} = (\mathbf{w}^{(C)}C)*\mathbf{u}^{k},
\end{equation}
where $\mathbf{w}^{(C)}\in\re^{3}$, thus the dimension of trainable weights remains unchanged. After training on the same data at $C=0.5$, this conditionally parameterized model is tested on both cases, and predicted the problem perfectly.

\begin{figure}
	\centering
	\subfloat[Training, $C=0.5$\label{fig diffusion C0.5}]{
    	\includegraphics[trim=10 25 10 40,clip,width=1\textwidth]{images/1d_diffusion/Contour_0.5_1.png}}\\
	\subfloat[Testing, $C=0.125$\label{fig diffusion C0.125}]{
    	\includegraphics[trim=10 25 10 40,clip,width=1\textwidth]{images/1d_diffusion/Contour_0.125_1.png}}
	\caption{1D diffusion: standard convolution (conv) vs conditionally parameterized convolution (cp-conv)} 
\end{figure} 



==> bak/2d_burgers.tex <==
\subsection{2D Viscous Burgers}
The 2D viscous Burgers equation is an example where we can fit the governing equation exactly with a conditionally parameterized network. It is clearly realized that for such type of problems, the use of deep learning is questionable. This test case is supposed to only serve as a idealized demonstration. 

With periodic boundary conditions, the equation is given by:

\begin{equation}\label{eq burgers}
\begin{split}
    &\frac{\partial u}{\partial t} + u\frac{\partial u}{\partial x} + v\frac{\partial u}{\partial y} - \nu(\frac{\partial^2 u}{\partial x^2}+\frac{\partial^2 u}{\partial y^2})=0,\\
    &\frac{\partial v}{\partial t} + u\frac{\partial v}{\partial x} + v\frac{\partial v}{\partial y} - \nu(\frac{\partial^2 v}{\partial x^2}+\frac{\partial^2 v}{\partial y^2})=0,\\
    &x\in[0,W], y\in[0,H], t\in[0,T],\\
    &\mathbf{u}(0,y,t)=\mathbf{u}(W,y,t), \mathbf{u}(x,0,t)=\mathbf{u}(x,H,t),
\end{split}
\end{equation}
% $\mathbf{u}=\begin{bmatrix}u\\v\end{bmatrix}$
where $\mathbf{u}=[u, v]^T$. It must be pointed out that the set-up for this test problem is a slightly modified copy of that from Ref.~\cite{geneva2020modeling}. The initial condition is determined by a spatially periodic function $\mathbf{g}$:
\begin{equation}
\begin{split}
    &\mathbf{g}(x,y) = \sum_{i=-L}^L\sum_{i=-L}^L\mathbf{a}_{ij}\sin(2\pi(ix+jy))+\mathbf{b}_{ij}\cos(2\pi(ix+jy)),\\
    &\mathbf{u}(x,y,0)=\frac{2\mathbf{g}(x,y)}{\max_{\{x,y\}}|\mathbf{g}(x,y)|}+\mathbf{c},
\end{split}
\end{equation}
where $\{\mathbf{a}_{ij}, \mathbf{b}_{ij}\}\sim \mathcal{N}(\mathbf{0},\boldsymbol{I}_2), L=4, \mathbf{c}\sim\mathcal{U}(-1,1)\in\re^2.$

With a forward in time and central in space discretization, the discretized form of \eqr{eq burgers} is:
\begin{equation}\label{eq burgers discrete}
\begin{split}
    &\frac{\Delta u^k_{i,j}}{\Delta t}+
    u^k_{i,j}\frac{u^k_{i+1,j}-u^k_{i-1,j}}{2\Delta x}+
    v^k_{i,j}\frac{u^k_{i,j+1}-u^k_{i,j-1}}{2\Delta y}
    -\nu\frac{u^k_{i-1,j}-2u^k_{i,j}+u^k_{i+1,j}}{\Delta x^2}
    -\nu\frac{u^k_{i,j-1}-2u^k_{i,j}+u^k_{i,j+1}}{\Delta y^2}=0,\\
    &\frac{\Delta v^k_{i,j}}{\Delta t}+
    u^k_{i,j}\frac{v^k_{i+1,j}-v^k_{i-1,j}}{2\Delta x}+
    v^k_{i,j}\frac{v^k_{i,j+1}-v^k_{i,j-1}}{2\Delta y}
    -\nu\frac{v^k_{i-1,j}-2v^k_{i,j}+v^k_{i+1,j}}{\Delta x^2}
    -\nu\frac{v^k_{i,j-1}-2v^k_{i,j}+v^k_{i,j+1}}{\Delta y^2}=0,
\end{split}
\end{equation}
where $i$ and $j$ are the grid indices in the $x$ and $y$ directions, respectively.

\eqr{eq burgers discrete} can be rewritten as:
\begin{equation}\label{eq burgers discrete2}
\begin{split}
    \Delta \mathbf{u}^k_{i,j}=&
    p_1(\mathbf{u}^k_{i+1,j}-\mathbf{u}^k_{i-1,j})
    +p_2(\mathbf{u}^k_{i,j+1}-\mathbf{u}^k_{i,j-1})+\\
    &p_3(\mathbf{u}^k_{i-1,j}-2\mathbf{u}^k_{i,j}+\mathbf{u}^k_{i+1,j})
    +p_4(\mathbf{u}^k_{i,j-1}-2\mathbf{u}^k_{i,j}+\mathbf{u}^k_{i,j+1}),
\end{split}
\end{equation}
where $p_1=-\frac{\Delta t}{2\Delta x}u^k_{i,j}, p_2=-\frac{\Delta t}{2\Delta y}v^k_{i,j}, p_3=\nu\frac{\Delta t}{\Delta x^2}, p_4=\nu\frac{\Delta t}{\Delta y^2}.$

Due to the nonlinear terms, e.g. $p_1(\mathbf{u}^k_{i+1,j}-\mathbf{u}^k_{i-1,j})$, \eqr{eq burgers discrete2} cannot be fitted by a simple CNN. Instead, by using  $p_{\{1,2,3,4\}}$ as parameters to a conditionally parameterized CNN (CP-CNN), the equation can be fitted exactly: 
\begin{equation}\label{eq burgers cpconv}
    \Delta \mathbf{u}^{k} = (\mathbf{w}_1p_1)*\mathbf{u}^{k}+
    (\mathbf{w}_2p_2)*\mathbf{u}^{k}+
    (\mathbf{w}_3p_3)*\mathbf{u}^{k}+
    (\mathbf{w}_4p_4)*\mathbf{u}^{k},
\end{equation}
where $\{\mathbf{w}_1, \mathbf{w}_3\}\in\re^{2\times3\times1\times2}, \{\mathbf{w}_2, \mathbf{w}_4\}\in\re^{2\times1\times3\times2}.$

In common deep learning applications, the models can rarely fit the truth exactly, thus a large amount of training data is needed to train the model sufficiently and to avoid overfitting. However in this test case, we expect the model to be fitted exactly to the truth, thus minimal training data is needed and overfitting is no longer a problem for predictions as the governing equation remains consistent. 

To demonstrate this, we use only 3 pairs of training data, each for a different set of parameters $\nu, \Delta x, \Delta y$, to train a model represented by \eqr{eq burgers cpconv}. Each pair of them only has one snapshot of initial condition $\mathbf{u}^0$ as the input, and the solution for $\Delta \mathbf{u}^0$ as the target output. All training data is present in Fig.~\ref{fig burgers training}. 
% In Table~\ref{table burgers params}, the trained parameters for different terms in \eqr{eq burgers cpconv} are compared with the desired values to match \eqr{eq burgers discrete}. It can be seen that they matches closely.

The model is used to perform roll-out prediction for 100 steps at a new initial condition and set of parameters outside the training range, $\nu=0.015, \Delta x=0.016, \Delta y=0.016$. The result is present in Fig.~\ref{fig burgers testing}. The L1 error is less than \num{1e-4}. 

In comparison, standard CNN represented by \eqr{eq burgers cnn} is used for the same task with a 3-by-3 kernel with 2 channels, $\mathbf{w}\inr{3\times 3\times 2\times 2}$. The total trainable parameters in the standard CNN is 36 compared with 24 for the CP-CNN. It can be seen that the CNN cannot predict the dynamics correctly, and some values grow to infinity due to insufficient prediction of diffusion.

\begin{equation}\label{eq burgers cnn}
    \Delta \mathbf{u}^{k} = \mathbf{w}*\mathbf{u}^{k}.
\end{equation}

\begin{figure}
	\centering
	\subfloat[$\nu=0.01, \Delta x=0.02, \Delta y=0.02$]{
    	\includegraphics[width=0.33\textwidth]{images/2d_burgers/Train_Contour_0.png}}
	\subfloat[$\nu=0.012, \Delta x=0.03, \Delta y=0.02$]{
    	\includegraphics[width=0.33\textwidth]{images/2d_burgers/Train_Contour_1.png}}
	\subfloat[$\nu=0.012, \Delta x=0.02, \Delta y=0.03$]{
    	\includegraphics[width=0.33\textwidth]{images/2d_burgers/Train_Contour_2.png}}
	\caption{2D Viscous Burgers: 3 groups of training data, each being only the one-step solution for a different IC and set of parameters. Top: $\mathbf{u}^0$; bottom: $\Delta\mathbf{u}^0$} \label{fig burgers training}
\end{figure} 


\begin{figure}
	\centering
	\includegraphics[trim=75 65 0 85,clip,width=0.95\textwidth]{images/2d_burgers/CNN_Contour_3.png}
	\caption{2D Viscous Burgers: prediction result on a new IC and set of parameters, $\nu=0.015, \Delta x=0.016, \Delta y=0.016$. From top to bottom: truth, CP-CNN prediction, CNN prediction; row 1 to 3: $u$, row 4 to 6: $v$} \label{fig burgers testing}
\end{figure} 

% \begin{table}[!ht]
% 	\begin{center}
% 	\caption {2D viscous Burgers: trained parameters}\label{table burgers params}
% 	\begin{tabular}{c| c c}
% 	\hline
% 	Parameter & Desired & Trained\\
% 	\hline
% 	$\mathbf{w}_1$ & $[0.5, 0, -0.5]^T$& $[0.499995, 0.00001, -0.500005]^T$\\
% 	$\mathbf{w}_2$ & $[0.5, 0, -0.5]$& $[0.5000004, -0.0000006, -0.4999993]$\\
% 	$\mathbf{w}_3$ & $[1, -2, 1]^T$& $[0.99993, -1.99990,  0.99993]^T$\\
% 	$\mathbf{w}_4$ & $[1, -2, 1]$& $[1.00006, -2.0001,  1.00006]$\\
% 	\hline
% 	\end{tabular}
% 	\end{center}  
% \end{table}

==> bak/2d_injector_old.tex <==
\subsection{Rocket Engine Injector}
The Deepblue\footnote{\url{https://afcoe.engin.umich.edu/benchmark-data}} is a public dataset generated from a high-fidelity simulation for the combustion process in a truncated rocket engine injector. Solutions are provided on a finite-volume mesh of $n_x=38523$ cells for eight primitive variables $$\mathbf{q}=[p, v_x, v_y, T, Y_{\text{CH4}}, Y_{\text{O2}}, Y_{\text{H2O}}, Y_{\text{CO4}}]^T,$$ where $p$ is the pressure, $v_x$ and $v_y$ are the $x$ and $y$ velocity components, $T$ is the temperature and \{$Y_{\text{CH4}}, Y_{\text{O2}}, Y_{\text{H2O}}, Y_{\text{CO4}}$\} are the mass fractions for the four chemical species involved in the combustion process. The simulation is performed using the finite-volume based General
Equation and Mesh Solver (GEMS), where the residual $R$ for a set of conservative variables $\mathbf{q}_c=[\rho, \rho v_x, \rho v_y, \rho e, \rho Y_{\text{CH4}}, \rho Y_{\text{O2}}, \rho Y_{\text{H2O}}, \rho Y_{\text{CO4}}]$ are first solved, and then converted to the change in $q$ using a Jacobian matrix $\mathbf{\Gamma}=\partial \mathbf{q}/\partial \mathbf{q}_c$. The governing equation can be written as:
\begin{align}
    \frac{\delta \mathbf{q}}{\delta t}= \mathbf{\Gamma r},\\
    \mathbf{r} = -\nabla(\mathbf{k-k}_{\nu})+\mathbf{s},
\end{align}
where $\mathbf{k}$ is the inviscid flux term, $\mathbf{k}_{\nu}$ is the viscous flux term and $\mathbf{s}$ is the source term. A detailed description to the dataset and simulation can be found in \cite{mcquarrie2020data}.

In this work, we try to perform a deep-learning based prediction for $\mathbf{q}$. The goal is to develop a neural network operator $g$ such that 
\begin{equation}
    \Delta \mq^t=g(\mq^t, \Delta \mq^{t-1}),
\end{equation}
where $t$ is the time step index and $\Delta q^t=q^{t+1}-q^t$ is change of $q$ between step $t+1$ and $t$. 

% Describe finite volume RHS and inversion computation

% To develop $g$ on the original unstructured CFD mesh, a graph neural network (GNN) model is necessary. However, a standard GNN does not take account of the topology features such as the relative direction and distance between nodes, which are of vital importance in a CFD problem. Thus we developed a conditionally parameterized GNN based on the edge conditioned convolution (ECC) architecture.

We follow the framework introduced in Sec.~\ref{sec cpnet}, with a few modifications. In this test, the nodes of the graph are defined on the cell centers,  with node features being the cell-averaged solution variables plus the inverse of pressure. I.e. for a cell with index $i$, the node feature is $\mathbf{x}_i = [\mathbf{q}_i; 1/p_i]$
% \begin{equation}
    % n_i = [p_i, v_{x,i}, v_{y,i}, T_i, Y_{\text{CH4},i}, Y_{\text{O2},i}, Y_{\text{H2O},i}, Y_{\tex\mathbf{k}t{CO4},i}, 1/p_i.
% \end{equation}

The adjacency relation of nodes are determined based on a 9-point stencil, i.e. each node, as a center, is connected to its immediate upper, lower, left, right, upper-left, upper-right, lower-left and lower-right neighbors. 

The neural network $G$ consists of two types of layers, namely the dense layer $D$ and the conditionally parameterized dense layer $D_{cp}$, the operations of which can be written as:
\begin{align}
    D(x)=\mathbf{w}x+b,\\
    D_{cp}(x,p)=(\mathbf{w}p+b_1)x+b_2,
\end{align}
where $x$ is the input feature, $p$ is the input parameter, $\mathbf{w}$ and $b$ are the trainable weights and biases. 

The architecture of $G$ can be separate into three blocks: a leading feature extraction block of $D_{cp}$ layers that generates high order hidden representations from inputs followed by two parallel residual computation blocks of different reception fields that predicts the residual of different physical scales, respectively. The output of the two residual blocks are summed up into the final output $\Delta q$. 

The feature extraction block can be formulated as:
\begin{align}
    n0_i=D_{cp}(q^k_i, q^k_i),\\
    n1_i=D_{cp}(h0_i, h0_i),\\
    n2_i=D_{cp}(q^k_i, q^k_i),\\
    n3_i=D_{cp}(h0_i, h0_i),\\
    e0_{i,j}=D_{cp}(e_{i,j}, e_{i,j}),\\
    e1_{i,j}=D_{cp}(e_{i,j}, e_{i,j}),\\
    e2_{i,j}=D_{cp}(n2_j, e1_{i,j}),\\
    e2_{i,i}=D_{cp}(n2_i, 0),
\end{align}
where $n$ and $e$ are hidden variables on nodes and edges, respectively. 

The first residual computation block with the smaller reception field can be formulated as:
\begin{align}
    f0_i=\sum_{j\in N(i)}[D_{cp}(h1_i-h1_j,e0_{i,j})+D_{cp}(h1_i+h1_j,e0_{i,j})],\\
    f1_i=\sum_{j\in N(i)}[D_{cp}(f0_i-f0_j,e0_{i,j})+D_{cp}(f0_i+f0_j,e0_{i,j})].
\end{align}

The other residual computation block with the larger reception can be formulated as:
\begin{align}
    g0_i=\sum_{j\in N(i)\cup i}[D_{cp}(\Delta q^{k-1}_j,e2_{i,j})],\\
    g1_i=\sum_{j\in N(i)\cup i}[D_{cp}(\Delta g0_j,e2_{i,j})],\\
    g2_i=\sum_{j\in N(i)\cup i}[D_{cp}(\Delta g1_j,e2_{i,j})],\\
    g3_i=\sum_{j\in N(i)\cup i}[D_{cp}(\Delta g2_j,e2_{i,j})].
\end{align}
The final output is computed as:
\begin{equation}
    y_i=D_{cp}(f1_i, n3_i)+D(g3_i).
\end{equation}
Since the output $y^k=G(q^k,\Delta q^{k-1},e)$ is the prediction for $\Delta q^k$, more future steps can be predicted recurrently as:
\begin{equation}
\begin{split}
q^{k+l}=q^{k+l-1}+y^{k+l-1},\\
\Delta y^{k+l}=G(q^{k+l},y^{k+l-1},e).
\end{split}
\end{equation}

In the numerical test, the simulation result is sampled at a time interval of \num{1e-6} s. Five sampled steps are used for training, and prediction is performed for the next 75 steps. The results for 4 variables, $p, v_x, T, Y_{\text{CH4}}$,are provided in Fig.~\ref{fig injector contour}. 

\begin{figure}
	\centering
	\subfloat[$k=0$ (initial condition)]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 0,clip,width=1\textwidth]{images/deepblue/prediction/pressure_0.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 0,clip,width=1\textwidth]{images/deepblue/prediction/u_0.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 0,clip,width=1\textwidth]{images/deepblue/prediction/t_0.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 0,clip,width=1\textwidth]{images/deepblue/prediction/ch4_0.png}
    	\end{minipage}
    }\\
	\subfloat[$k=5$ (end of training)]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/pressure_5.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/u_5.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/t_5.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/ch4_5.png}
    	\end{minipage}
    }\\
	\subfloat[$k=10$]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/pressure_10.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/u_10.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/t_10.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/ch4_10.png}
    	\end{minipage}
    }\\
	\subfloat[$k=15$]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/pressure_15.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/u_15.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/t_15.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/ch4_15.png}
    	\end{minipage}
    }\\
	\subfloat[$k=25$]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/pressure_25.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/u_25.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/t_25.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/ch4_25.png}
    	\end{minipage}
    }\\
	\subfloat[$k=50$]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/pressure_50.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/u_50.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/t_50.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/ch4_50.png}
    	\end{minipage}
    }\\
	\subfloat[$k=75$]{
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/pressure_75.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/u_75.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/t_75.png}
    	\end{minipage}
    	\begin{minipage}{0.25\linewidth}
    	\includegraphics[trim=230 40 210 150,clip,width=1\textwidth]{images/deepblue/prediction/ch4_75.png}
    	\end{minipage}
    }
	\caption{Prediction results. From left to right: $p, v_x, T, Y_{\text{CH4}}$}\label{fig injector contour} 
\end{figure} 
% results

==> bak/introduction_old.tex <==
\section{Introduction}
The simulation of complex fluid dynamics and physics has been indispensable in many scientific and industrial fields. The need for more accurate and efficient models for this task leads to the use of machine learning and data-driven methods to improve or replace traditional numerical methods that are mainly based on the solution of partial differential equations (PDEs). The  tremendous successes of neural networks in the computer science field have recently boosted extensive explorations in applying and adjusting them to the physics modeling tasks. In such explorations occurred numerous developments in the network architectures and learning methods, many of which target to impose constraints and information developed from existing governing equations into the construction of neural networks. 

Projection-based methods are one of the most popular application of machine learning in the physics computation field. Such methods first construct a low-dimensional subspace, on which computations are performed for a set of reduced order variables in order to reduce the total degrees of freedom in the system. Early projection-based method commonly rely on a linear subspace constructed using the proper orthogonal decomposition (POD)~\cite{berkooz1993proper, rowley2004model}, and a formal projection of the original governing equations via Galerkin formulations, which has been applied successfully to complex problems such as turbulent flows~\cite{rowley2005model, carlberg2011efficient,hijazi2019data} and combustion instabilities~\cite{xu2019reduced, huang2018exploration}. Recently, autoencoder networks have become a popular alternative to the POD, due to its capability of generating a non-linear set of projection basis as well as providing more flexibility in the desired properties to be learned, thus bringing improvements in both efficiency and predictive capabilities~\cite{hartman2017deep,guo2016convolutional,puligilla2018deep,carlberg2019recovering,lee2018model, murata2020nonlinear}. The Galerkin computation of reduced variables can also be replaced by surrogate models build from regression models~\cite{hesthaven2018non, wang2019non,  san2019artificial}, auto-regressive models such as recurrent neural networks (RNN)~\cite{rumelhart1988learning, gonzalez2018deep, maulik2020reduced}, long-short term memory networks (LSTM)~\cite{hochreiter1997lstm, mohan2019compressed, maulik2020time}, temporal convolutional networks (TCN)~\cite{xu2020multi} or inferred equations~\cite{brunton2016discovering, kramer2019nonlinear, kramer2019balanced}. 

Another family of machine learning applications on the top of traditional PDE-based computational methods is to improve the accuracy and reliability of existing models or solutions via parameter inference~\cite{yarlanki2012estimation}, uncertainty quantification~\cite{dow2011quantification, tracey2013application, xiao2016quantifying} and model augmentation~\cite{singh2017machine, duraisamy2015new, wu2018physics}, super-resolution~\cite{wang2012proper, fukami2021machine, pradhan2020super, guo2020ssr}, etc.

A substantial difference between tasks in the computational physics field and other popular machine learning tasks is the availability of governing equations, which are usually in the form of PDEs. In physics-informed neural networks (PINN)~\cite{raissi2019physics}, the violation of physics, quantified by the residual of the governing PDEs, is included as a regularization term in the loss function in the training process. PINN has been shown to sufficiently reduce the required amount of labeled training data~\cite{raissi2019physics}. With proper treatment of the boundary and initial conditions, even data-free training can be realized~\cite{sun2020surrogate}. Although the PINN is originally proposed for fully-connected networks, the idea has also been successfully incorporated into other network architectures such as convolutional neural networks (CNN) ~\cite{gao2020phygeonet}.

The CNN has long been the most popular choice for processing large-scale spatially distributed data. A important reason is its weight-sharing property, which significantly reduces the training cost, as well as enables it to capture local features, thus providing better predictive performances especially for travelling dynamics. However standard CNNs can only work with problems discretized on a Euclidean space, represented by a uniform linear/rectangular/cuboid mesh, which largely restricts its application on complex geometries and multi-scale physics. Encoded geometric labels e.g. signed distance function (SDF)~\cite{guo2016convolutional, bhatnagar2019prediction}, and more mathematically formal treatments e.g. elliptic coordinate transformation~\cite{gao2020phygeonet} have been used to alleviate this restriction. However, they are still bounded to meshes with quadrilateral cells and require additional pre-processing of the geometric information, which is often difficult to be automated. The graph convolutional network (GCN)~\cite{kipf2016semi} and more generally, the graph neural networks (GNN) work directly on non-uniform grids, and thus become a natural alternative to CNN for CFD applications. GNNs have demonstrated extraordinary performances in both particle-based~\cite{sanchez2020learning} and mesh-based simulations~\cite{pfaff2020learning, belbute2020combining}.

The aforementioned improvements are mostly focused on selecting most the suitable form of loss function and layers to utilize existing prior knowledge and data structure. In this work, we try to apply the idea of conditional parametrization to the CFD field, which is a modification within network layers than can potentially be applied to any existing architectures. 





